On the "Naturalness" of Buggy Code

Real software, the kind working programmers produce by the kLOC to solve real-world problems, tends to be "natural", like speech or natural language; it tends to be highly repetitive and predictable. Researchers have captured this naturalness of software through statistical models and used them to good effect in suggestion engines, porting tools, coding standards checkers, and idiom miners. This suggests that code that appears improbable, or surprising, to a good statistical language model is "unnatural" in some sense, and thus possibly suspicious. In this paper, we investigate this hypothesis. We consider a large corpus of bug fix commits (ca.~8,296), from 10 different Java projects, and we focus on its language statistics, evaluating the naturalness of buggy code and the corresponding fixes. We find that code with bugs tends to be more entropic (i.e., unnatural), becoming less so as bugs are fixed. Focusing on highly entropic lines is similar in cost-effectiveness to some well-known static bug finders (PMD, FindBugs) and ordering warnings from these bug finders using an entropy measure improves the cost-effectiveness of inspecting code implicated in warnings. This suggests that entropy may be a valid language-independent and simple way to complement the effectiveness of PMD or FindBugs, and that search-based bug-fixing methods may benefit from using entropy both for fault-localization and searching for fixes.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
# DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> tables/context_diff.tex <==
% Table generated by Excel2LaTeX from sheet 'context_diff.csv'
\begin{table*}[!htbp]
 % \centering
  \scriptsize
    \begin{tabular}{lrrrrr}
    \toprule
     project         & thr = 2  & thr = 5 & thr = 10 & thr = 20 & thr = 30 \\
    \midrule
    Atmosphere  & 1.12 to 1.87  & 0.94 to 1.36   & 0.76 to 1.08   & 0.40 to 0.66   & 0.42 to 0.66 \\
    Derby            & 1.59 to 2.19  & 1.69 to 2.03   & 1.41 to 1.65   & 1.12 to 1.31   & 0.96 to 1.13 \\
    OpenJPA       & 1.86 to 2.68  & 1.47 to 1.91   & 1.24 to 1.57   & 1.04 to 1.31   & 0.97 to 1.21 \\
    Elasticsearch & 1.62 to 2.17  & 1.48 to 1.74   & 1.14 to 1.34   & 0.98 to 1.14   & 0.87 to 1.01 \\
    Facebook      & 0.49 to 1.88  & 1.17 to 1.99   & 0.91 to 1.55   & 0.95 to 1.45   & 0.84 to 1.28 \\
    Lucene          & 1.07 to 1.99  & 0.87 to 1.37   & 0.77 to 1.13   & 0.93 to 1.21   & 0.76 to 1.02 \\
    Presto           & 0.96 to 1.95  & 0.88 to 1.44   & 0.84 to 1.26   & 0.73 to 1.08   & 0.71 to 1.01 \\
    Netty            & 1.89 to 2.39  & 1.57 to 1.85   & 1.34 to 1.55   & 1.16 to 1.33   & 1.02 to 1.17 \\
    Qpid              & 1.41 to 2.09  & 1.32 to 1.68   & 1.16 to 1.41   & 0.85 to 1.05   & 0.78 to 0.95 \\
    Wicket          & 1.63 to 2.19  & 1.60 to 1.93   & 1.36 to 1.61   & 1.15 to 1.35   & 1.12 to 1.31 \\
    \midrule
    Average                 & 1.78 to 2.01  & 1.55 to 1.67   & 1.29 to 1.37   & 1.07 to 1.14   & 0.97 to 1.03 \\
    \bottomrule
    \end{tabular}%
    \caption{95\% confidence interval of the difference between CDE of buggy lines vs.~non-buggy lines reported by t-test. Wilcox non-parametric test confirmed buggy lines higher CDE than non-buggy lines with statistical significance. `thr' represents the maximum number of lines deleted in a change. The result shows with 95\% confidence that buggy lines have 0.97 to 1.03  bit higher entropy than non-buggy lines while considering all the changed. However, for smaller change size buggy lines have 1.78 to 2.01 bit higher CDE than non-buggy lines.}
  \label{tab:ld}%
\end{table*}%

